MedInsight: A Multi-Source Context Augmentation Framework for Generating Patient-Centric Medical Responses using Large Language Models

Large Language Models (LLMs) have shown impressive capabilities in generating human-like responses. However, their lack of domain-specific knowledge limits their applicability in healthcare settings, where contextual and comprehensive responses are vital. To address this challenge and enable the generation of patient-centric responses that are contextually relevant and comprehensive, we propose MedInsight:a novel retrieval augmented framework that augments LLM inputs (prompts) with relevant background information from multiple sources. MedInsight extracts pertinent details from the patient's medical record or consultation transcript. It then integrates information from authoritative medical textbooks and curated web resources based on the patient's health history and condition. By constructing an augmented context combining the patient's record with relevant medical knowledge, MedInsight generates enriched, patient-specific responses tailored for healthcare applications such as diagnosis, treatment recommendations, or patient education. Experiments on the MTSamples dataset validate MedInsight's effectiveness in generating contextually appropriate medical responses. Quantitative evaluation using the Ragas metric and TruLens for answer similarity and answer correctness demonstrates the model's efficacy. Furthermore, human evaluation studies involving Subject Matter Expert (SMEs) confirm MedInsight's utility, with moderate inter-rater agreement on the relevance and correctness of the generated responses.

==> context_length.tex <==
%A pre-defined context length is typically used to pre-train large language models \cite{chen2023longlora}. As it is obvious, using long context to train LLMs seems to be expensive for many researchers. Various works have been conducted with the aim of extending context length \cite{chen2023longlora}.  LongLoRA has been presented in \cite{chen2023longlora} as an efficient model for fine-tuning being useful for the context size extension of pre-trained LLMs. This approach provides limited computation cost since training large language models with long context sizes require extensive GPU and more training hours causing expensive computational cost. Then Yang presented another effective model called LongQLoRA for extending the context length of LLMs \cite{yang2023longqlora}.  This method is memory efficient, and it requires less training sources working based on the combination of Position Interpolation \cite{chen2023extending}, QLoRA \cite{dettmers2023qlora} and Shift Short Attention \cite{chen2023longlora} of LongLoRA. Using LongQLoRA the context length of LLaMA2 has been extended from 4096 to 8192. Position Interpolation (PI) has been presented to extend the context window sizes for several pre-trained large language models. In this approach, the aim is that the max position index needs to be matched to the previous context window \cite{chen2023extending}. To do so, the position indices are downscaled and there was no need to use extrapolation in this method. 

%In a study conducted by Dettmers et al., another efficient finetuning technique called QLORA has been introduced. This approach reduces memory usage efficiently on a single 48GB GPU and it also preserve the full finetuning task performance. Equipped with NF4, double quantization and paged optimizers, QLORA can save memory effectively while preserving the full performances \cite{dettmers2023qlora}. Shift short (an efficient finetuning method) has been introduced in \cite{chen2023longlora}  as a local attention mechanism splitting the tokens into different groups and then computes the attention individually in every single group. Additionally, it can compute the attention among the adjacent groups to provide better information interaction among neighboring groups. SelfExtend based approach has been presented in \cite{jin2024llm} to stimulate LLMs’ long context. The main idea behind this approach is constructing bi-level attention information, namely: the neighbor level and the group level. Original model’s self-attention helps to ease the computation of these levels. This means that the proposed method does not necessarily need any training.Position encoding works well in transformer architecture and for dependency modeling among different elements at various sequences’ positions. Rotary Position Embedding (RoPE) has been proposed in \cite{su2024roformer} to leverage the positional information efficiently. One of the desirable properties for NL coding is that RoPE decays once the relative distance increases, so we can consider this as one of the profitable properties of rotary position embedding \cite{su2024roformer}.  Although transformers adapt well for some tasks like natural language processing, their expressive power is still agnostic \cite{yun2019transformers}. There are several research in literature focusing on position encoding into the learning phase. 

%Parkish et al., \cite{parikh2016decomposable} presented a simple neural architecture for NLP. This technique works based on an attention for decomposing the problem into several separate subproblems; and then make it trivially parallelizable. An algorithm to reduce the intermediate memory requirement of some existing approaches to linear in the sequence length has been developed in \cite{huang2018music} enabling us to prove that a modified relative attention mechanism-based Transformer would be able to easily produce minute-long compositions. Shaw et al. \cite{shaw2018self} introduced an alternative approach, to extend the self-attention mechanism to consider the relative positions’ representations and distances among seq components effectively. In another study, a neural architecture Transformer-XL enabling learning dependency beyond a fixed length has been proposed to resolve issues related to context fragmentation as well as longer term dependencies \cite{dai2019transformer}. Yang et al., presented a generalized autoregressive pre-training approach called XLNet \cite{yang2019xlnet}. This technique equipped with maximizing the expected likelihood over all factorization’s permutations order enables learning bidirectional contexts. More importantly, BERT’s existing limitations are resolved using XLNet’s autoregressive formulation. 

%Apart from the above mentioned studies, there are also several recent works focusing on position encoding and attention mechanism \cite{su2024roformer}.The landscape of transfer learning methods for natural language processing has been presented in \cite{raffel2020exploring}. In this work, a unified framework converting all text-based language problems into a text-to-text format has been introduced. Additionally, architectures, pre-training objectives, transfer approaches, and unlabeled data sets have been compared and analyzed on various tasks related to language understanding.Ke et al., investigated the positional encoding approaches utilized in language pre-training. Additionally, several problems have been identified in the existing formulations. In this study, a new positional encoding method (Transformer with Untied Positional Encoding (TUPE)) has been presented \cite{ke2020rethinking}. In this approach, the positional correlation and word contextual correlation are computed separately with different parameterizations and then are added together.In another study Huang et al., \cite{huang2020improve} argued that position information cannot be fully utilized in the existing works. It is obvious that the sinusoid embedding’s initial proposal is fixed and is not learnable. Motivated by this drawback, new approaches encouraging the interaction between query, key and relative position embeddings in the self-attention mechanism have been presented in \cite{huang2020improve}. The performance of various natural language processing tasks has been improved remarkably with the advancements in neural language models. In this paper we propose a new architecture called DeBERTa (Decoding-enhanced BERT with disentangled attention) has been developed by He et al., \cite{he2020deberta} to enhance the performance of BERT and RoBERTa techniques utilizing two new methods.

%Transformers on the other hand can identify complex dependencies among various components of each sequence \cite{choromanski2020rethinking}. They are considered as powerful Neural NET models providing promising results and outcomes in solving various real-world problems. Various studies have been introduced for context length extension of transformers. To name a few, Karpukhin et al., indicated that retrieval may be done suing dense representation itself \cite{karpukhin2020dense}, and Izacard et al., \cite{izacard2022few} introduced a new RAG model to understand and learn knowledge tasks using only a few training samples. In another study conducted by Gunn et al., the efficiency of retrieval augmented language models has been demonstrated with fine tuning of Open-QA’s challenging tasks \cite{guu2020retrieval}. In these methods language models are augmented through including related documents and the retrieved results into contexts. 

%There are some researches in the literature focused on modifying multi-head attention. In these studies, the self-attention computations’ quadratic complexity has been alleviated. Wang et al., \cite{wang2020linformer} developed informer, a self-attention mechanism with linear complexity.  In this study, the authors realized that self-attention may be approximated by a low-rank matrix, and it can also reduce the overall complexity in time and space. 
%As it is obvious, transformers cannot process long sequences because of their self-attention mechanism scaling quadratically with the sequence length. To solve this issue, Beltagy et al., \cite{beltagy2020longformer} introduced longformer. This long document transformer uses an attention mechanism scaling linearly with sequence length. Reformer has also been presented in another study conducted by Kitaev et al., \cite{kitaev2020reformer} as a memory efficient method with faster processing ability on long contexts. The quadratic dependency on the context length is one of the critical drawbacks of transformer techniques. To tackle this issue, a new approach which works based on a sparse attention with the aim of reducing this dependency has been introduced in \cite{zaheer2020big}. Additionally, memory augmented transformer has been developed in \cite{bulatov2022recurrent} to resolve the issue related to the complexity of self-attention mechanism due to the quadratic computation. 

%Pretrained Language Models such as RoBERTa \cite{liu2019roberta} and BERT \cite{devlin2018bert} were very common and popular in natural language processing before developing large language models. Lacking robustness, difficulty in explanation, and the need for extremely large amount of data were among important barriers and impediments that PLMs faced \cite{he2023survey}. 
%Recent progress and advancements of LLMs and its ability in efficiently responding to free-text queries and it’s significant performance in healthcare domain equipped with professional knowledge have improved these areas and created both concern and excitement \cite{he2023survey}. Many researches have been conducted to apply LLM in healthcare showing promising results in various tasks such as Relation Extraction (RE), medical Named Entity Recognition (NER), and Semantic Textual Similarity (STS) \cite{kalyan2022ammu} \cite{he2023survey}.

%Nowadays we can also see more practical applications of AI based methods combined with LLM in healthcare such as answering patients and clinical questions in the hospital \cite{he2023survey} \cite{chen2023benchmark} \cite{shi2023midmed}, automatic multimodal medical report generation \cite{moon2022multi}. In \cite{chen2023benchmark} authors developed two approaches for supporting medical consultation (understanding the doctor–patient dialogue and task-oriented interaction). Lack of medical knowledge became one of the important challenges for patients to determine their main goals. In this case, MidMed as a new approach creating a human-human medical consultation dialogue, has been developed \cite{shi2023midmed}. This task covers five types of dialogue such as knowledge-grounded dialogue, task-oriented, recommendation, chitchat, and QA.
%Additionally, Medical Vision Language Learner (MedViLL) has been conducted in a study proposed by \cite{moon2022multi}. This method combined BERT architecture with a multi-modal attention masking scheme for enhancing and maximizing the generalization performance for tasks related to vision-language understanding and vision-language generation. 


% \subsection{Large Language Models}
% \label{large_language_models}
% Human language can be comprehended and generated by some computational techniques like Large Language Models (LLMs) \cite{chang2023survey}. These LLMs are mainly transformer-based techniques which consists of an encoder  and decoder which can be trained on various types of text-based datasets containing huge number of parameters. The self-attention mechanism in the Transformer's \cite{vaswani2017attention} architecture is considered as the main part of various LLMs like GPT-4 \footnote{OpenAI, GPT-4, Website: openai.com/research/gpt-4}, LLAMA2 \cite{touvron2023llama} and PaLM \cite{chowdhery2023palm}. Fast and exceptional learning abilities, accurate natural language understanding and comprehension, and other tasks such as generating response and providing answers to questions are among the important benefits of Large Language Models.

% The Natural Language Processing (NLP) is a sub-field in AI which leverage various learning-based algorithms enabling machines to fully understand human languages. Currently, LLMs using transformers can easily perform tasks related to natural language processing with high accuracy. Existing Large Language Models can employ either encoder only (BERT, RoBERTa), decoder only (GPT2, GPT3), or encoder-decoder (BART) transformers and pre-training models. These models can be trained \textit{autoregressively} i.e., \textit{predicting the next word based on the given left-hand context}, or by \textit{masking}  i.e., \textit{predicting the masked words based on the given context on both sides}, or \textit{corrupting a sequence and then predicting the original sequence}. Capturing long dependencies in text, handling sequential data effectively, facilitating parallelization are also possible by the above mentioned architectures. 

% In-context learning or prompting is among the the crucial features and characteristics of Large Language Models \cite{brown2020language}. It is the practice of incorporating natural language text into the input or output to encourage the LLM to generate text based on the given context or prompt enabling large languages to provide accurate, coherent and contextually relevant responses. Moreover, users will be engaged in question-response interactions with LLMs %, posing questions to the model and receiving answers %, thereby engaging in a natural language conversation 
% \cite{chang2023survey}. 


% \subsection{Retrieval Augmented Generation} Pre-trained Large Languages can acquire detailed and extensive knowledge from {training} data \cite{ petroni2019language}. %These model learns This learning occurs without the need for access to external memory, serving as a parameterized implicit knowledge base \cite{raffel2020exploring}. 
% However, there maybe some pitfalls for these models: they are not able to expand their memory or revise and may potentially generate \textit{hallucinations}~\cite{ji2023survey}. Hybrid methods that combine %parametric memory with non-parametric (i.e., retrieval-based) memories 
%     {global knowledge inherent to LLM and local knowledge database relevant to an organization} have been presented to tackle these types of issues. Retrieval Augmented Generation (RAG) is one of those methods \cite{lewis2020retrieval}. In the following paragraphs, we will discuss briefly about a general formulation of RAG.% and explore its key components.
    
%     Some tasks such as text generation are conceptualized as a mapping from an input sequence $l$ to an output sequence $q$, formulated as $q=f(l)$. For instance, in dialogue response generation, $l$ and $q$ can be denoted as the dialogue history. % and its corresponding response, while in machine translation, they could represent the text in the source language and its translation in the target language. %\input{table_deifnation_CTI} 
%     %Recently, some researchers \cite{guu2020retrieval, lewis2020retrieval} have proposed enhancing LLMs with the ability to access external data source through information retrieval techniques. This augmentation allows models to gather relevant information during the generation process. 
%     In Retrieval Augmented Generation (RAG), the user input sequence $l$ can be leveraged by the models for retrieving the text passages $z$ from %an external document corpus
%     a local database. The passages which are retrieved successfully can be incorporated as an additional context while generating the target sequence $q$. Note that, the retriever, represented as as $p_n(z|l)$ with parameters $n$, outputs the top-k chunks of text passages in response to query $l$. 
    
%  We further explore the usage of modern Natural Language Processing (NLP) techniques in the realm of healthcare as follows.


% The global knowledge retrieval system employs agents to perform web searches based on user prompts, following a systematic approach known as "thoughts, action, and observation." This process relies on reputable sources such as WebMD or Mayo Clinic for extracting clinical information. Within agents, a language model serves as a reasoning engine, guiding the decision-making process to determine the sequence and order of actions to be taken. Agents are equipped with tools, which are interfaces enabling interactions with the external environment. These tools function as aids for agents to carry out various actions, including web searches, database searches, code execution, calculations, and API calls. In our specific context, the tool facilitates web searches in response to user queries. For instance, when presented with the user prompt mentioned earlier, the following sequence unfolds: \textit{{\fontfamily{qcr}\selectfont \textbf{Thought:} "It is imperative to possess a comprehensive understanding of the condition before delving into its effects." \textbf{Action:} Search WebMD, \textbf{Action Input:} Kawasaki disease, \textbf{Observation:} "Kawasaki disease is a very rare and mysterious ailment that strikes children under age 5. The symptoms include a high … If your child is showing symptoms of Kawasaki disease, … seek medical attention immediately."}}
